Validating a novel angular power spectrum estimator using simulated low frequency radio-interferometric data

The "Tapered Gridded Estimator" (TGE) is a novel way to directly estimate the angular power spectrum from radio-interferometric visibility data that reduces the computation by efficiently gridding the data, consistently removes the noise bias, and suppresses the foreground contamination to a large extent by tapering the primary beam response through an appropriate convolution in the visibility domain. Here we demonstrate the effectiveness of TGE in recovering the diffuse emission power spectrum through numerical simulations. We present details of the simulation used to generate low frequency visibility data for sky model with extragalactic compact radio sources and diffuse Galactic synchrotron emission. We then use different imaging strategies to identify the most effective option of point source subtraction and to study the underlying diffuse emission. Finally, we apply TGE to the residual data to measure the angular power spectrum, and assess the impact of incomplete point source subtraction in recovering the input power spectrum $C_{\ell}$ of the synchrotron emission. This estimator is found to successfully recovers the $C_{\ell}$ of input model from the residual visibility data. These results are relevant for measuring the diffuse emission like the Galactic synchrotron emission. It is also an important step towards characterizing and removing both diffuse and compact foreground emission in order to detect the redshifted $21\, {\rm cm}$ signal from the Epoch of Reionization.

==> readme <==
%auto-ignore

This file contain information regarding the paper "Validating a novel angular power spectrum estimator using simulated low frequency radio-interferometric data"

Authors:Samir Choudhuri, Nirupam Roy , Somnath Bharadwaj, Sk. Saiyad Ali, Abhik Ghosh and H.T. Intema, and

Comments: 18 pages, 1 table, 9 figures, Accepted for publication in New Astronomy Journal.

The contact details of the first author are as follows
Samir Choudhuri
email  : samir11@phy.iitkgp.ernet.in
Address: Indian Institute of Technology Kharagpur
         Kharagpur-721302, India



Abstract:
The ``Tapered Gridded Estimator'' (TGE) is a novel way to directly estimate the 
angular power spectrum from radio-interferometric visibility data that reduces 
the computation by efficiently gridding the data, consistently removes the 
noise bias, and suppresses the foreground contamination to a large extent by 
tapering the primary beam response through an appropriate convolution in the 
visibility domain. Here we demonstrate the effectiveness of TGE in recovering 
the diffuse emission power spectrum through numerical simulations. We present 
details of the simulation used to generate low frequency visibility data for 
sky model with extragalactic compact radio sources and diffuse Galactic synchrotron emission. We then use different imaging strategies to identify the most effective option of point source subtraction and to study the underlying diffuse emission. Finally, we 
apply TGE to the residual data to measure the angular power spectrum, and 
assess the impact of incomplete point source subtraction in recovering the 
input power spectrum $C_{\ell}$ of the synchrotron emission. This estimator is 
found to successfully recovers the $C_{\ell}$ of input model from the residual 
visibility data. These results are relevant for measuring the diffuse emission like 
the Galactic synchrotron emission. It is also an important step towards 
characterizing and removing both diffuse and compact foreground emission in 
order to detect the redshifted $21\, {\rm cm}$ signal from the Epoch of 
Reionization.

